Multichannel Long-Term Streaming Neural Speech Enhancement for Static and Moving Speakers

In this work, we extend our previously proposed offline SpatialNet for long-term streaming multichannel speech enhancement in both static and moving speaker scenarios. SpatialNet exploits spatial information, such as the spatial/steering direction of speech, for discriminating between target speech and interferences, and achieved outstanding performance. The core of SpatialNet is a narrow-band self-attention module used for learning the temporal dynamic of spatial vectors. Towards long-term streaming speech enhancement, we propose to replace the offline self-attention network with online networks that have linear inference complexity w.r.t signal length and meanwhile maintain the capability of learning long-term information. Three variants are developed based on (i) masked self-attention, (ii) Retention, a self-attention variant with linear inference complexity, and (iii) Mamba, a structured-state-space-based RNN-like network. Moreover, we investigate the length extrapolation ability of different networks, namely test on signals that are much longer than training signals, and propose a short-signal training plus long-signal fine-tuning strategy, which largely improves the length extrapolation ability of the networks within limited training time. Overall, the proposed online SpatialNet achieves outstanding speech enhancement performance for long audio streams, and for both static and moving speakers. The proposed method is open-sourced in https://github.com/Audio-WestlakeU/NBSS.

==> coverletter-R1.tex <==
\begin{coverletter}{Multichannel Long-Term Streaming Neural Speech Enhancement for Static and Moving Speakers}{SPL-39066-2024}


\begin{answereditor}{Based on the attached set of reviews, I reach the conclusion that the paper can be accepted, but that certain minor revisions are necessary (giving this an "AQ" status, ACCEPTED WITH MANDATORY CHANGES), as follows:

I hope that you will carefully consider these comments and take necessary actions. Your revised manuscript must be uploaded within 2 (TWO) weeks to your account in Manuscript Central (https://mc.manuscriptcentral.com/spl-ieee).}

We keenly thank the four reviewers for the efforts they provided in the evaluation of our paper. Based on the reviewers' comments we prepared a revised manuscript. The major revisions are the followings:
\begin{itemize}
 \item We provided all the clarifications required or suggested by the reviewers. 
 \item We fixed all the typos pointed out by the reviewers.
 \item We added more details about the dataset as suggested by the reviewers.
 
 % provided all the clarifications required or suggested by the reviewers. 
 % \item An additional experiment is added to evaluate the extent to which the proposed SpatialNet relies on spectral information for both six-channel and single-channel cases. 
 % \item The computational cost and model size of the proposed SpatialNet are compared with the involved  baseline methods.
 % \item A new ASR is used, and the corresponding new results are reported.  
 % \item Experiments with various SNRs are added.
 % \item The batch mode WPE method is experimentally compared. 
 % \item The ASR results for the dynamic dataset are added.
\end{itemize}

In a general manner, we took care to address all the concerns of the four reviewers. Please find below our detailed answers to the reviewers' questions and comments.
\textbf{An annotated version of the revised manuscript, in which the modifications, novel paragraphs and sections are highlighted in green and numbered R1, R2, etc., is attached at the end of this cover letter. Our detailed answers below refer to these annotations, e.g., ``Revision\#4 on P4'' means that annotation R4 can be found on Page 4 of the attached revised manuscript}. 

\end{answereditor}

\begin{answerreviewer}[AQ - Publish In Minor, Required Changes]

\qa{The authors extend the offline SpatialNet for long-term streaming multichannel speech enhancement in both static and moving speaker scenarios. The main novelty is the proposed three variants of oSpatialNet as well as the ST+LF strategy. Although this work is only evaluated on simulated datasets, the details (e.g. the 6-channel microphone array and real-recorded noise signals from CHiME3, clean speech signals from the WSJ0 corpus) indicate that it may achieve a good performance on real datasets.

The paper is well written and easy to follow, I have only a few minor comments below.}
{
Thank you for these positive comments, we have revised the paper concerning all of your comments as follows.
}

\qa{
1. 1st paragraph in Section II "...conducts time convolution (with a kernel size of 5)..." I suggest it could be replaced by "...conducts convolution with a kernel size of 1 and 5 on the frequency and time axes, respectively" for readers to understand easier, since the convolution is operated in T-F domain.
}{
We have revised this according to your suggestion see \refcm{tfconv}.
}


\qa{
2. Section II Retention part. "...O(1) inference cost for each time step..." I think the letter O should be italic.
}{
According to your suggestion, this has been revised see \refcm{italicO}.
}

\qa{
3. Section III-A. How are the parameters chosen? e.g. the room size, the moving speed. Is it selected according to other papers, corpus, or some real application scenarios? What tools are used for simulating the dataset? In my opinion, since this work is trained and evaluated on simulated datasets, the details above should be provided to make the results more convincing.
}{
Thank you for your suggestion. We have revised our paper see \refcm{gpurir}, \refcm{speed} and \refcm{train-test-diff}. For the parameters of room size, we follow our previous work [13].

% The parameters are chosen following some previous works, e.g. [13] and [31], see \refcm{speed}. The tool used for simulation is gpuRIR see \refcm{gpurir}. More details  
}

\qa{
4. 1st paragraph in Section III-C. I understand that the same amount of training utterances are used. But do the 3 models get converged? Since the LT(32s,36e) gets better performance than LT(32s,18e) when using oSpatialNet-MSA and oSpatialNet-Ret, can they achieve better performance if more epochs are trained?
}{
The three models, including oSpatialNet-MSA and oSpatialNet-Ret, are almost converged when the training strategy LT(32s,36e) is used, and training these models with more epochs won't change the conclusions in the paper. This is clarified in the revised manuscript, please see \refcm{converge}.
}

\qa{
5. Conclusion "Three variants have be developed..." A grammar mistake.
}{
Thanks for pointing out this, it is corrected in the revised manuscript.
}

\end{answerreviewer}


\begin{answerreviewer}[AQ - Publish In Minor, Required Changes]

\qa{
1. The best results in Table I should be highlighted.
}{
Thank you for this suggestion. The best results in Table I have been highlighted in the revised manuscript.
}

\qa{
2. Why did a sudden performance drop happen around the 60s in Fig.2?
}{
Thank you for pointing out this issue. After careful examination, we found that the issue arises because the generated speech signals around 58 s have a slightly higher input SISNR (about 0.2 dB) than other segments, which brings a sudden performance increase in around 58 s and a sudden performance drop afterward. In addition, we think there is a slight inaccuracy of performance measuring at the end of the signal due to the signal truncation. Therefore, we think the sudden performance drop is not caused by any intrinsic properties of the models.
% Consequently, a steep increase in performance around 58 s occurs, which, in turn, creates the illusion of a sudden performance drop for subsequent speech segments. Further examination has confirmed that this issue exists in all baseline methods compared in the paper. Hence, it won't undermine the validity or impartiality of the reported results.
}

\qa{
3. Another common scenario is the position sudden change. Did the authors have the corresponding experimental results?
}{
Thank you for this valuable comment. The position sudden change is an important scenario in real-life, but this paper doesn't study this scenario and focuses on the static and moving speakers scenarios. We will study this important scenario in the future.
}
\end{answerreviewer}

\begin{answerreviewer}[AQ - Publish In Minor, Required Changes]
    
\qa{
The authors propose a modification of their previously introduced architecture SpatialNet to facilitate online speech enhancement of long sequences. Three architectural choices to replace a regular self-attention module are examined: masked self-attention, retention and Mamba (state-space model). The goal is to achieve linear time-complexity and good exploitation of long-term dependencies. The authors explicitly evaluate the performance for long input sequences and show that problems exist, but they can easily be fixed by fine-tuning on longer sequences.
}{
Thanks for your comments. We have revised the paper concerning all of your comments as follows.
}

\qa{
Why are 8 kHz chosen as a sampling rate? To me this is a rather outdated choice which also weakens the validity of all experiments. Both CHiME3 and WSJ0 have been recorded in 16 kHz, which I would consider the minimum sampling rate today.
}{
Indeed, 16 kHz sample rate is widely used and considered as the minimum sample rate by many applications. In this paper, 8 kHz sample rate is used for two reasons: a) the models can be trained much faster under 8 kHz sample rate than a higher sample rate, e.g. 16 kHz; b) our preliminary experiments revealed that the models behave similarly for 8 kHz and 16 kHz. This has been briefly explained in the revised manuscript, see \refcm{sf}. 
% Consequently, the choice of 8 kHz sample rate in this paper won't affect the validity of our experiments.
}

\qa{
The performance evaluation with respect to the signal length is quite interesting. I was not aware that there is a problem evaluating on longer sequences than those used during training. I have never noticed this for architectures that use LSTMs for sequence modelling, but also never thoroughly tested it. I think, for completeness, it would be good to also include a baseline which uses a classical LSTM for the narrowband sequence modeling. This way, all the modern and often chosen architectures for sequence modeling would be part of the comparison.
}{
Thank you for the suggestion. Due to the page limitation, we did not present the network architectures of McNet and EaBNet in the previous manuscript. Actually, both of them have LSTM/GRU sub-networks for the narrowband sequence modeling. Thus the paper indeed includes the results of all the modern and often chosen architectures as you suggested.

% According to their papers, EaBNet [36] is composed of convolutional layers and GRU layers, while McNet [16] is composed of LSTM layers. The GRU layers in EaBNet and one of the LSTM layers in McNet both work in narrowband. Both of them achieve outstanding performance compared to many modern baselines, so they can be considered as 

% The baseline methods, i.e. McNet and EaBNet, both have narrowband LSTM/GRU sub-networks. They can be considered as 
% {
% \centering
%   \includegraphics[width=0.4\linewidth]{r64s_eabnet_mcnet.png}
%    \vspace{-0.8cm}
%   \caption{Speech enhancement performance for different training strategies.}
% }

% \begin{figure}[htbp]
  % \centering
  % \includegraphics[width=0.4\textwidth]{r64s_eabnet_mcnet.png}
  % \caption{Speech enhancement performance of EaBNet$^+$ and McNet for different training strategies}
  % \label{fig:your_figure_label}
% \end{figure}

}

\qa{
The best performance is obtained with offline SpatialNet. I guess this is expected since it is non-causal? Please give an explicit explanation.
}{
Yes, this is because the offline SpatialNet is non-causal and leverages some future information. This is clarified in the revised manuscript, see \refcm{noncausal}.
% it can obtain better estimation of the spatial characteristics of noise, reverberation and direct-path speech. Consequently, a better performance on the dereverberation and denoising task (the task of this paper) can be obtained.
% The offline SpatialNet obtained the best performance since it is non-causal so that 
}

\qa{
The paper compares different modern architectural choices for narrow-band sequence modeling in an online setting. The most interesting part is the evaluation showing that problems with long sequences can be fixed by using some long sequences for fine-tuning. I think an LSTM baseline should be added to Figure 2 to make the comparison of sequence modeling techniques more complete. I would then recommend to accept the paper.
}{
Thank you for your suggestion. As mentioned in our response to your previous comment, both McNet and EaBNet involve LSTM/GRU subnetworks for the narrowband sequence modeling. In the below figure, we show the results of McNet and EaBNet as a function of signal time. It seems that, when trained with short signals (4s), both the networks have certain length extrapolation problem, especially for the moving speaker case, but not as severe as the proposed models. After finetuning with long signals (32 s), McNet learns to properly use the information provided by longer signals, while the performance of EaBNet is entirely improved.  
% As shown in the figure, the two networks trained with short signals (4s) have slight, e.g. EaBNet$^+$ ST(4s) in moving speaker case, or almost don't have length extrapolation problem. After long signal fine-tuning (LF), both of two networks achieved better performance, where for McNet, its ability to leverage more historic information is enhanced, while for EaBNet, besides of that, its ability to conduct speech enhancement at beginning stage is also enhanced. 
We agree with reviewer that these results are interesting, and we will dive deeper in the future. However, we really cannot add these results in the paper due to the page limitation. 

% its ability for modeling long term information is increased, while for EaBNet, its 

% almost don't have any length extrapolation problem in both moving and static speaker scenarios even trained with signals much shorter than the test signals, i.e. EaBNet$^+$ ST(4s) and McNet ST(4s).

\includegraphics[width=0.4\textwidth]{r64s_eabnet_mcnet.png}
}

\qa{
TYPOS:
I. Introduction, first paragraph
Most of these methods in literature assumes -$>$ assume

II. Online SpatialNet, Part B
In most of -$>$ In most

II. Online SpatialNet, Part B
Academic researches -$>$ academic research

II. Online SpatialNet, Part B
Training with long signals is benefit -$>$ beneficial
}{
Thank you for pointing out the typos. These typos are corrected in the revised manuscript see \refcm{assume}, \refcm{most}, \refcm{research}, and \refcm{beneficial}.
}


\end{answerreviewer}


\begin{answerreviewer}[AQ - Publish In Minor, Required Changes]
    

\qa{
The paper is very well written and structured.
While the evaluation is only on sythetic signals, this is ok for a more theoretically oriented SPL. The main information missing is how the test set differs from the training set.
}{
Thanks for your positive comments. The training set and test set are generated in the same way. The only difference between the two sets is the utterance length, see \refcm{train-test-diff}.
}


\end{answerreviewer}

\end{coverletter}

\twocolumn
\setcounter{page}{1}
\setcounter{figure}{0}
